A Family-Based Approach to Safety Cases for Controlled Airspaces in Small Uncrewed Aerial Systems

As small Uncrewed Aircraft Systems (sUAS) increasingly operate in the national airspace, safety concerns arise due to a corresponding rise in reported airspace violations and incidents, highlighting the need for a safe mechanism for sUAS entry control to manage the potential overload. This paper presents work toward our aim of establishing automated, customized safety-claim support for managing on-entry requests from sUAS to enter controlled airspace. We describe our approach, Safety Case Software Product Line Engineering (SafeSPLE), which is a novel method to extend product-family techniques to on-entry safety cases. It begins with a hazard analysis and design of a safety case feature model defining key points in variation, followed by the creation of a parameterized safety case. We use these together to automate the generation of instances for specific sUAS. Finally we use a case study to demonstrate that the SafeSPLE method can be used to facilitate creation of safety cases for specific flights.

==> paper.tex <==
\section{From Abstract to Paper}

If accepted to submit a full paper, we will extend our abstract to a full paper reporting on an example to demonstrate the construction of an initial, partial feature model of sUAS features and constraints, its transformation into a parameterized safety case, and results from its experimental use to generate sUAS-specific safety-case instances.  We also will explore integration of results from our safety-case product line with the broader infrastructure that determines whether to allow or deny entry to a sUAS.   





==> related.tex <==
\section{Related Work}
